OpenXAI: Towards a Transparent Evaluation of Model Explanations

While several types of post hoc explanation methods have been proposed in recent literature, there is very little work on systematically benchmarking these methods. Here, we introduce OpenXAI, a comprehensive and extensible open-source framework for evaluating and benchmarking post hoc explanation methods. OpenXAI comprises of the following key components: (i) a flexible synthetic data generator and a collection of diverse real-world datasets, pre-trained models, and state-of-the-art feature attribution methods, and (ii) open-source implementations of eleven quantitative metrics for evaluating faithfulness, stability (robustness), and fairness of explanation methods, in turn providing comparisons of several explanation methods across a wide variety of metrics, models, and datasets. OpenXAI is easily extensible, as users can readily evaluate custom explanation methods and incorporate them into our leaderboards. Overall, OpenXAI provides an automated end-to-end pipeline that not only simplifies and standardizes the evaluation of post hoc explanation methods, but also promotes transparency and reproducibility in benchmarking these methods. While the first release of OpenXAI supports only tabular datasets, the explanation methods and metrics that we consider are general enough to be applicable to other data modalities. OpenXAI datasets and models, implementations of state-of-the-art explanation methods and evaluation metrics, are publicly available at this GitHub link.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec:overview} for a step-by-step justification of \name's contributions and Section~\ref{sec:expt} for an in-depth benchmarking analysis of explanation methods using our \name framework.}
  \item Did you describe the limitations of your work?
    \answerYes{In Section~\ref{sec:overview} we discuss that \name includes only six datasets and seven post-hoc explainers in its current release. However, we provide detailed instructions on how users can leverage our easy-to-use class templates and add new datasets and explainers to our pipeline. In addition, we discuss how \name ameliorates the limitation of previous benchmarks by providing the first-ever public leaderboard for comparing post-hoc explainers.
    }
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{ }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Appendix~\ref{app:datasets},~\ref{app:model},~\ref{app:parameter} for a detailed description about the dataset, data splits, model architectures (number of layers, activation function, etc.), hyperparameter details of the post-hoc explainers, and metric settings. In addition, we open-source our codes in the \href{https://github.com/AI4LIFE-GROUP/OpenXAI}{\name} GitHub repository. To improve the accessibility, interoperability, and reuse of ML tools, we apply \href{https://github.com/force11/FAIR4RS}{FAIR4RS principles and implementation} guidelines to all software and ML tools included in \name. We strongly believe that software and ML tools should be open and adhere to FAIR principles to encourage repeatability, reproducibility, and reuse.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{app:exp} for all training details.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Figures~\ref{fig:german_disparity_lr}-\ref{fig:adult_disparity_lr} where we report the error bars that denote the error in the metric performance across all instances in the test set.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{app:model} for the compute used in benchmarking \name's post-hoc explainers.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{All assets, including datasets, post-hoc explainers, and evaluation metrics are properly cited.}
  \item Did you mention the license of the assets?
  \answerYes{MIT License.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> overflow.tex <==

% \begin{minipage}[c]{0.47\textwidth}
%     \centering\small
%     \renewcommand{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{1.8pt}
%     \captionof{table}{
%         Summary of currently available feature attribution methods in \name. “Learning?” denotes whether learning/training procedures are required to generate explanations and "White-box Access?" denotes if the access to the internals of the model (e.g., gradients) are needed %if the underlying model are treated as a white- (\cmark) or black-box (\xmark) during the explanation stage.
%         % “Flow” denotes the computational flow used by the feature attribution method for generating explanations, 
%         % and “Design” indicates whether an explanation method has specific design requirements. \chirag{remove design}
%     }    
%     {\begin{tabular}{lcccc}
%     \toprule
%     % Method TYPE LEARNING TASK TARGET BLACK-BOX FLOW DESIGN
%     {Method} & {Learning?} & {White-box Access?} \\ % & {Design} \\ % & {Flow} % & {RRS} & {ROS} & {Fairness} \\
%     \toprule
%     \begin{tabular}[l]{@{}l@{}}{Random}\\{\Grads}\\{\IntGrad}\\{\GradtimesInput}\\{\SmoothGrad}\\{\SHAP}\\{\LIME}
%     \end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}
%         \xmark\\
%         \xmark\\
%         \xmark\\
%         \xmark\\
%         \xmark\\
%         \cmark\\
%         \cmark\\
%     \end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}
%         \xmark\\
%         \cmark\\
%         \cmark\\
%         \cmark\\
%         \cmark\\
%         \xmark\\
%         \xmark\\
%     \end{tabular} \\
%     % \begin{tabular}[c]{@{}c@{}}
%     %     Forward\\
%     %     Backward\\
%     %     Backward\\
%     %     Backward\\
%     %     Backward\\
%     %     Forward\\
%     %     Forward\\
%     % \end{tabular} &
%     % \begin{tabular}[c]{@{}c@{}}
%     %     \xmark\\
%     %     \xmark\\
%     %     \cmark\\
%     %     \xmark\\
%     %     \cmark\\
%     %     \cmark\\
%     %     \cmark\\
%     % \end{tabular} \\    
%     \bottomrule \\
%     \end{tabular}}
%     \label{tab:explanation}
% \end{minipage}
% \quad
% \begin{minipage}[c]{0.45\textwidth}
% \centering\small
% \begin{mdframed}[hidealllines=true,backgroundcolor=blue!10]
% \textcolor{violet}{@abstractmethod}\\
% \textcolor{orange}{def} \textcolor{violet}{get\_explanations}(self, model, X: torch.\textcolor{brown}{Tensor}, y: torch.\textcolor{brown}{Tensor}):\\
% \textcolor{gray!75}{~~~~"""}\\\
%     \textcolor{gray!75}{~~~~Generate explanations for given input/s.}\\
%     \textcolor{gray!75}{~~~~Parameters}\\
%     \textcolor{gray!75}{~~~~------------------------}\\
%     \textcolor{gray!75}{~~~~model: pre-trained ML model}\\
%     \textcolor{gray!75}{~~~~X: torch.tensor}\\
%         \textcolor{gray!75}{~~~~~~~~Input in two-dimensional shape (m, n).}\\
%     \textcolor{gray!75}{~~~~y: torch.tensor}\\
%         \textcolor{gray!75}{~~~~~~~~Labels}\\
%     \textcolor{gray!75}{~~~~Returns}\\
%     \textcolor{gray!75}{~~~~------------------------}\\
%     \textcolor{gray!75}{~~~~torch.Tensor}\\
%         \textcolor{gray!75}{~~~~~~~~Explanation vector/matrix.}\\
%     \textcolor{gray!75}{~~~~"""}\\
%     \textcolor{orange}{~~~~pass}
% \end{mdframed}
% % \renewcommand{\arraystretch}{1.2}
% % \setlength{\tabcolsep}{1.8pt}
% % \captionof{figure}{\name Python package: All resources in \name, including data loaders, data processing helpers, explanation methods, predictor model, and evaluation metrics can be easily accessed via our Python package. 
% % % The \name package is installed using PyPI package management system. 
% % Here, we first create a DataLoader object and use it to obtain a dataset. The second block shows how to access the pre-trained ML model. The third and fourth code blocks illustrate how to benchmark the performance of an explanation method for a given metric. See our GitHub repository and website for more details.}
% % \includegraphics[width=0.99\textwidth]{paper/neurips_benchmark/FIG/openxai_library_code.pdf}
% % \label{tab:german_stab_lr}
% \end{minipage}

\hima{Satya to make a pass by 4pm ET today; Related work in main paper can be a couple of paragraphs and thats it. No need to reiterate stuff already in the intro.}
\emph{Post hoc Explanations}: Several techniques have been proposed in recent literature to construct \emph{post hoc explanations} of complex models. These techniques differ in their access to the complex model (i.e., black box vs. access to internals), scope of approximation (e.g., global vs. local), search technique (e.g., perturbation-based vs. gradient-based), and basic units of explanation (e.g., feature importance vs. rule-based). 
For instance, LIME, SHAP, Anchors, BayesLIME and BayesSHAP~\cite{ribeiro16:model-agnostic,lundberg17:a-unified,slack2021reliable,ribeiro2018anchors} are \emph{perturbation based local} explanations as they leverage perturbations of individual instances to construct interpretable local approximations (e.g., linear models), which in turn serve as explanations of individual model predictions. 
On the other hand, methods such as \GradtimesInput, \SmoothGrad, \IntGrad, and GradCAM~\cite{simonyan2013saliency, sundararajan2017axiomatic, selvaraju2017grad,smilkov2017smoothgrad} are \emph{gradient based local} explanations as they leverage gradients computed with respect to input dimensions of individual instances to explain model predictions. An alternate class of methods known as \emph{global} explanations attempts to summarize the behavior of black box models as a whole~\cite{bastani2017interpretability,lakkaraju19:faithful,kim2017interpretability}. 
 %rather than in relation to individual data points%(see \cite{arrieta2020explainable, guidotti2018survey, murdoch2019definitions, linardatos2021explainable,covert2021explaining} for surveys). 
%In contrast, our work focuses on analyzing the disagreements between explanations generated by state-of-the-art methods. 

\emph{Evaluating Post hoc Explanations}: \hima{need to chop pieces below and clean up text}
Prior research has studied several notions of explanation quality such as fidelity, stability, consistency and sparsity~\cite{liu2021synthetic,petsiuk2018rise,slack2021reliable,zhou2021evaluating}. %Several metrics to quantify each of these aspects of explanation quality were also proposed~\cite{zhou2021evaluating,carvalho2019machine,gilpin2018explaining,liu2021synthetic}.
Several metrics are proposed to determine if an explanation is reliable~\cite{zhou2021evaluating,carvalho2019machine,gilpin2018explaining,liu2021synthetic}. An extensive survey of metrics for evaluating explanation methods can be found in \citet{zhou2021evaluating}, who propose two high-level goals of explanation methods: interpretability (the clarity, simplicity, and broadness of the explanations), and fidelity (the completeness and soundness of explanations)~\cite{carvalho2019machine, gilpin2018explaining}. 
%e.g., \citet{liu2021synthetic} provide a synthetic benchmark for explanation evaluation which includes implementations of several metrics, as well as a discussion of how to choose metrics for evaluation. As discussed earlier, 
%However, they rely on the unrealistic assumption of the availability of ground truth explanations. 
There are also metrics for evaluating explanation aspects such as fidelity, stability, consistency, and sparsity~\cite{liu2021synthetic,petsiuk2018rise,slack2021reliable,zhou2021evaluating,ghorbani2019interpretation,alvarez2018robustness,hooker2018evaluating,lakkaraju19:faithful}. 
For instance, \citet{hooker2018evaluating} proposed ``Remove and Retrain'' (ROAR), which measures the fidelity of an explanation by retraining the model with and without the features deemed as most important by the explanation. However, it may not always be feasible to retrain the underlying model.
~\citet{lakkaraju19:faithful} measured fidelity by comparing the predictions of the underlying model with those produced by the explanation (linear model). This approach works only for the case where the explanation and the underlying model are both predictive models. 
Follow up works leveraged these properties and metrics to
theoretically and empirically analyze the behavior of popular post hoc explanations~\cite{ghorbani2019interpretation, slack2019can,dombrowski2019explanations,adebayo2018sanity,alvarez2018robustness,levine2019certifiably,pmlr-v119-chalasani20a,agarwal2021towards}.
More specifically it has been shown that these explanations can be inconsistent or unstable \cite{ghorbani2019interpretation, slack2019can}, prone to fair washing~\cite{lakkaraju2020fool,slack2019can,aivodji2019fairwashing}, and can be unfaithful to the model to the extent that their usefulness can be severely compromised~\cite{rudin2019stop}.
%demonstrated that methods such as LIME and SHAP may result in explanations that are not only inconsistent and unstable, but also prone to adversarial attacks. 

Another key vulnerability of explanations generated by state-of-the-art post hoc explanation methods is fair washing~\cite{lakkaraju2020fool,slack2019can,aivodji2019fairwashing}. 
More specifically,~\citet{lakkaraju2020fool} and~\citet{slack2019can} showed that explanations which do not accurately represent the importance of sensitive attributes (e.g., race, gender) could potentially mislead end users into believing that the underlying models are fair (when they are not)~\cite{lakkaraju2020fool,slack2019can,aivodji2019fairwashing}. This, in turn, could lead to the deployment of unfair models in critical real world applications.
%There is also some discussion about whether models which are not inherently interpretable ought to be used in high-stakes decisions at all; \citet{rudin2019stop} argues that post hoc explanations tend to be unfaithful to the model to the extent that their usefulness is severely compromised. 
%While the aforementioned works analyze the behavior of post hoc explanation methods and expose some of their vulnerabilities, 
%\hima{editing here} Recent work has shed light on the downsides of post hoc explanation techniques. For instance, \citet{rudin2019stop} argued that post hoc explanations are not reliable, as these explanations are not necessarily faithful to the underlying models and present correlations. There has also been recent work on empirically exploring vulnerabilities of black box explanations~\cite{adebayo2018sanity,slack2019can,lakkaraju2020how,rudin2019stop,dombrowski2019explanations}---e.g.,~\citet{ghorbani2019interpretation} demonstrated that post hoc explanations may not be robust, changing drastically even with small perturbations to inputs~\cite{alvarez2018robustness}. In addition to the above works, there has also been some recent research that focuses on theoretically analyzing the robustness~\cite{levine2019certifiably,pmlr-v119-chalasani20a}, and other properties~\cite{garreau2020looking} of some of the popular post hoc explanation techniques. However, these works do not attempt to explore deeper connections between different classes of these techniques. \hima{more about evaluation metrics}

\xhdr{Benchmarking the Quality of Post hoc Explanations}
\begin{enumerate}
    \item XAI-Bench is a library for benchmarking feature attribution explainability techniques~\citep{liu2021synthetic} -- e.g., \citet{liu2021synthetic} provide a synthetic benchmark for explanation evaluation which includes implementations of several metrics, as well as a discussion of how to choose metrics for evaluation. However, their work is not broadly applicable because real world datasets cannot be approximated by synthetica datasets. 
    \item Quantus -- provides open source implementations of mutiple evaluation metrics, however they do not focus on rigorous benchmarking and leaderboards, and their metrics also do not cover new notions of stability and fairness unlike ours. 
\end{enumerate}

\hide{
In this section, we provide an overview of the OpenXAI framework. This framework comprises of the following key components: i) datasets and explainers, ii) evaluation metrics, iii) a public leaderboard

\subsection{Datasets and Explainers}
\label{sec:dataset}

\name includes synthetic with ground-truth explanations and real-world datasets to benchmark the quality of any explanation method. Further, our comprehensive dataset class (described in Sec.~\ref{sec:design}) allows researchers and practitioners to integrate new datasets into \name. Below we describe few existing datasets from our library.

\subsubsection{Synthetic Dataset}
\label{sec:synthetic}

Using real-world datasets for evaluating explanations is non-trivial due to the lack of ground-truth explanations. In addition, for providing reasonable confidence in benchmarking synthetic datasets, it is critical to ensure that the synthetic graphs satisfy some key properties like unique explanations. Previous works have shown that even random baselines can obtain high faithfulness score for trivial ground truth explanations~\citep{}, which questions the effectiveness of the state-of-the-art explanation methods. To this end, we argue that \name needs a benchmarking dataset where a simple baseline (like random explanations~\citep{agarwal2021towards}) cannot detect the ground truth explanation. To this end, we propose \textit{SynthGauss} -- a synthetic dataset for benchmarking explanation methods that has unique ground-truth explanations. In the initial release of \name, we generate \textit{SynthGauss} using $N$ clusters such that $n \in \{1,\dots, N\}$. Without any loss of generality, we describe \textit{SynthGauss} using 2 classes such that $c \in \{1,2\}$, but the parameterization capability of \textit{SynthGauss} allows users to generate multi-class datasets.

Let $\mathbf{\mu}_n$ be a $d$-dimensional mean vector, and $\mathbf{\Sigma}_n$ the corresponding $d \times d$-dimensional covariance matrix. Further, let $\mathbf{m}_n \in \{0,1\}^d$ be a masking vector depending on the cluster assignment $n$. We denote the ground-truth vector of explanations $\mathbf{b}$ and consider the following data generating process for all samples $(\mathbf{x}_{i}, y_i)$.

After everything is set and done for all $i$, we find a threshold $\theta$ such that half of the samples belong to class 1 and the other half belong to class 2. This will yield the following tuple which our \textit{SynthGauss} dataset generator will return for every $i$:
\begin{equation}
    (\textup{cluster index, mask, label, explanation, masked explanation, input}) = (n, \mathbf{m}_n, y_i, \mathbf{b}, \mathbf{b} \odot \mathbf{m}_{n}, \mathbf{x}_{i})
\end{equation}

\hima{show dataloader example for synthgauss along with function parameters; assigned to chirag}
}
% \begin{equation}
%     \begin{split}
%         n & \sim  Cat(N) ~~~ \text{(Draw cluster index)} \\
%         \bx_i & \sim \mathcal{N}(\bmu_n, \bS_n) ~~ \text{(Draw Gaussian inputs)} \\
%         \pi_1 &= \Prob(Y=1) = \frac{\exp\big((\bb \odot \m_n)^T \bxi\big)}{1 + \sum_{c=1}^C \exp\big((\bb \odot \m_n)^T \bxi \big)} ~~~ \text{(Get class probabilities)} \\
%     \end{split}
%     \label{eq:gaussian_data_generation}
% \end{equation}
% After everything is set and done for all $i$, we find a threshold $\theta$ such that half of the samples belong to class 1 and the other half belong to class 2.
% This will yield the following tuple which our DGP function will return for every $i$:
% \begin{equation}
%     (\text{cluster idx, mask, class label, explanation, masked explanation, input vector}) = (n, \m_n, y_i, \bb, \bb \odot \m_n, \bxi).
% \end{equation}
\hide{

\subsubsection{Explainers}
a para about leveraging captum apis to have instances of different explanation methods. 

existing explainers 

new explainers 

\subsection{Evaluation metrics}
\label{sec:metrics}
Here, we describe different evaluation metrics that we included in the first iteration of \name. More specifically, we discuss various metrics (and their implementations) for evaluating the faithfulness, stability, and fairness of any given feature attribution method. While faithfulness metrics capture how well explanations mimic the underlying model, stability metrics measure robustness of explanations to input perturbations. Fairness metrics, on the other hand, measure group-based disparities in faithfulness or stability of explanations. OpenXAI is the first benchmark to incorporate metrics to evaluate all the three aforementioned notions of explanation reliability. 

\xhdr{Faithfulness} To measure how faithfully a given explanation mimics the underlying model, prior work has either leveraged synthetic datasets and models trained on them to obtain ground truth explanations or 

\hima{editing here} 
\emph{Ground-truth Faithfulness} The first set of evaluation metrics included in \name comprise of the six disagreement metrics proposed in \cite{krishna2022disagreement}, namely, Feature Agreement (FA), Rank Agreement (RA), Sign Agreement (SA), Signed Rank Agreement (SRA), Rank Correlation (RC), and Pairwise Rank Agreement (PRA). The disagreement metrics quantify i) the extent to which explanations differ in the top-$k$ features, the signs (or directions of contribution) and the ordering of these top-$k$ features, and ii) the extent to which explanations differ in the relative ordering of certain features of interest. While \citet{krishna2022disagreement} used the above metrics to quantify the disagreement between different explanation methods, \name leverages the metric to calculate the disagreement between ground-truth explanations (from synthetic datasets and logistic regression models) and explanations generated by explanation methods.

\emph{Predictive Faithfulness} With respect to faithfulness, \name includes two complementary metrics: i) Predictive Faithfulness (PF) which measures a decrease in the probability of the predicted class as important features are removed, where the importance is identified using an output explanation, and ii) Inverse Predictive Faithfulness (IPF) measures the increase in probability as important features are added to an empty feature set. For a given instance $\mathbf{x}$, we first obtain the prediction probability $\hat{y}$ output by the underlying model $f$, \ie $\hat{y}=f(\mathbf{x})$. Let $e_{\mathbf{x}}$ be an explanation for the model prediction of $\mathbf{x}$. We then generate a perturbed instance $\mathbf{x}'$ in the local neighborhood of $\mathbf{x}$ by keeping the original values of the top-$k$ features and sampling values for all the other features using some data distribution (\eg ground-truth data distribution, random distribution, uniform distribution or marginal distribution). Finally, we compute the prediction difference metric as:
\begin{equation}
    \Delta_{\textup{pred}}(\mathbf{x}, f, e_{\mathbf{x}}, k) = \mathbb{E}_{\mathbf{x}' \sim \textnormal{perturb($\mathbf{x}$, $e_{\mathbf{x}}$, $k$, $\mathcal{P}$)}}[|\hat{y} - f(\mathbf{x}')|],
    \label{eq:pred_preserve}
\end{equation}
where perturb($\cdot$) returns the noisy versions of $\mathbf{x}$ as described above. Note that $\mathcal{P}$ is used to instantiate a specific type of perturbation for sampling $\mathbf{x}'$. The difference between the prediction probabilities determine the quality of explanation with larger difference equivalent to worse explanation and vice-versa. Note that the local sampling and prediction preserve evaluation techniques enable us to ameliorate the problems of existing faithfulness metrics. In contrast to preserving the top-$k$ features, we can also generate a perturbed instance $\mathbf{x}'$ in the local neighborhood of $\mathbf{x}$ such that for all the top-$k$ features we sample values from some data distribution and keep the original values of the non-important features. For such cases, larger prediction difference (in Eqn.~\ref{eq:pred_preserve}) is equivalent to more faithful explanations.
% See Appendix~\citep{} for more details about the metric.

\xhdr{Relative Stability} 
% \hima{More info about original stability metric is needed}
\citet{alvarez2018robustness} formalize the first stability metric for feature-attribution methods, arguing that explanations should be robust to local perturbations of an input. To evaluate the stability of an explanation for instance $\mathbf{x}$, perturbed instances $\mathbf{x}'$ are generated by adding infinitesimally small noise to the clean instance $\mathbf{x}$ such that $\hat{y}_{\mathbf{x}} = \hat{y}_{\mathbf{x}'}$:
\begin{equation}
    \textup{S}(\mathbf{x},\mathbf{x}',\mathbf{e}_{\mathbf{x}},\mathbf{e}_{\mathbf{x}'}) = \max_{\mathbf{x}'} \frac{||~ \mathbf{e}_{\mathbf{x}}-\mathbf{e}_{\mathbf{x}'}~||}{||~\mathbf{x}-\mathbf{x}'~||}, ~\forall \mathbf{x}'~\textup{s.t.}~\mathbf{x}'\in\mathcal{N}_{\mathbf{x}};~\hat{y}_{\mathbf{x}}=\hat{y}_{\mathbf{x}'}
    \label{eq:old_stab1}
\end{equation}
where $\mathcal{N}_{\mathbf{x}}$ is a neighborhood of instances $\mathbf{x}'$ similar to $\mathbf{x}$, and $\mathbf{e}_{\mathbf{x}}$ and $\mathbf{e}_{\mathbf{x'}}$ denote the explanations corresponding to instances $\mathbf{x}$ and  $\mathbf{x}'$, respectively. In contrast to existing stability metrics which only assume black-box access to the predictive model,~\citet{agarwal2022rethinking} introduced Relative Stability that leverages model information to evaluate the stability of an explanation with respect to the change in the a) input data (Relative Input Stability (RIS)), b) intermediate representations (Relative Representation Stability (RRS)), and c) output logits of the underlying predictive model (Relative Output Stability (ROS)). To the best of our knowledge, \name is the first benchmark that hoards all the above stability metrics under the same library.

\xhdr{Fairness} A key property of explanation is to ensure that the quality of the resulting explanations is consistently high across various population subgroups including the minority groups. A disparity in explanations across subgroups can have serious ramifications, e.g., a domain expert can make worse decisions for a particular group because of a disparity in explanation quality. Here, we incorporate disparity measures from~\cite{dai2022fairness} for formulating the problem of detecting group-based disparities in explanation quality. In doing so, the metric measure disparities with respect to different aspects of explanation quality: disagreement disparity, faithfulness disparity, and stability disparity.


\hima{command for invoking evaluation metrics; }

\subsection{Leaderboard}

\hima{put a snapshot, this leaderboard is transparent evaluations. you can also order methods based on different aspects. }

\hima{how to include new methods in leaderboard }
}
% \begin{table}[h]
%     \centering\small
%     \renewcommand{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{2.5pt}
%     \caption{
%         \textbf{Summary of currently available datasets in \name.} Here, “feature types” denotes whether the feature is discrete (dis.) or continuous (cont.), “feature information” describes what kind of information is captured in the dataset, and “balanced” denotes whether the dataset is balanced w.r.t. the predictive label. % \hima{Chirag/Satya: fill the table; feature information means demographic information, criminal records, financial records, personal information; feature types is discrete or continuous or both}
%     }
%     {\begin{tabular}{lccccc}
%     \toprule
%     {Dataset} & {Size} & {\# of features} & {Feature types} & {Feature information} & {Balanced} \\
%     \toprule
%     \begin{tabular}[l]{@{}l@{}}{SynthGauss}\\{German~Credit~\cite{Dua:2019}} \\{HELOC~\cite{HELOC}}\\{COMPAS~\cite{jordan15:effect}}\\{Adult~Income~\cite{yeh2009comparisons}}\\{Give Me Some Credit~\cite{GiveMeCredit}}
%     \end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}
%         {5,000}\\
%         {1,000}\\
%         {9,871}\\
%         {18,876}\\
%         {48,842}\\
%         {102,209}\\
%     \end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}
%         {20}\\
%         {20}\\
%         {23}\\
%         {7}\\
%         {13}\\
%         {10}\\
%     \end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}
%         {continuous}\\
%         {discrete, continuous}\\
%         {continuous}\\ 
%         {discrete, continuous}\\
%         {discrete, continuous}\\
%         {discrete, continuous}\\
%     \end{tabular} &
%     \begin{tabular}[c]{@{}c@{}}
%         {synthetic}\\
%         {demographic, personal, financial}\\
%         {demographic, financial}\\
%         {demographic, personal, criminal}\\
%         {demographic, personal, education/employment, financial}\\
%         {demographic, personal, financial}\\
%     \end{tabular} &    
%     \begin{tabular}[c]{@{}c@{}}
%         {\cmark}\\
%         {\xmark}\\
%         {\cmark}\\
%         {\xmark}\\
%         {\xmark}\\
%         {\xmark}\\
%     \end{tabular} \\   
%     \bottomrule
%     \end{tabular}}
%     \label{tab:dataset}
% \end{table}
